Counterfactual Explanation with Multi-Agent Reinforcement Learning for Drug Target Prediction

Motivation: Many high-performance DTA models have been proposed, but they are mostly black-box and thus lack human interpretability. Explainable AI (XAI) can make DTA models more trustworthy, and can also enable scientists to distill biological knowledge from the models. Counterfactual explanation is one popular approach to explaining the behaviour of a deep neural network, which works by systematically answering the question "How would the model output change if the inputs were changed in this way?". Most counterfactual explanation methods only operate on single input data. It remains an open problem how to extend counterfactual-based XAI methods to DTA models, which have two inputs, one for drug and one for target, that also happen to be discrete in nature. Methods: We propose a multi-agent reinforcement learning framework, Multi-Agent Counterfactual Drug target binding Affinity (MACDA), to generate counterfactual explanations for the drug-protein complex. Our proposed framework provides human-interpretable counterfactual instances while optimizing both the input drug and target for counterfactual generation at the same time. Results: We benchmark the proposed MACDA framework using the Davis dataset and find that our framework produces more parsimonious explanations with no loss in explanation validity, as measured by encoding similarity and QED. We then present a case study involving ABL1 and Nilotinib to demonstrate how MACDA can explain the behaviour of a DTA model in the underlying substructure interaction between inputs in its prediction, revealing mechanisms that align with prior domain knowledge.

==> method_prelim.tex <==
%% LyX 2.3.3 created this file.  For more info, see http://www.lyx.org/.
%% Do not edit unless you really know what you are doing.

To provide the necessary technical background we briefly introduce Actor-Critic
Reinforcement learning (Sec.~\ref{sec:SingleAC}), and the general multi-agent reinforcement learning (MARL) (Sec.~\ref{sec:MARL}). 

\subsubsection{Actor-Critic RL}

\label{sec:SingleAC} \textbf{Actor-critic} In this learning framework,
the agent learns to maximize the expected discount returns over the
future $T$ steps: $J=\mathbb{E}\left[\sum_{t=1}^{T}\gamma^{t}r^{t}\right]$
for discount factor $\gamma\in[0,1]$. To optimize the agent policy
with respects to the expected discount returns, the gradient is estimated
as: 
\begin{equation}
\nabla_{\theta}J(\pi_{\theta})=\nabla_{\theta}\log\pi_{\theta}(a_{t}|s_{t})R(t)
\end{equation}
where $R(t)=\sum_{t'=T}^{\infty}\gamma^{t'-t}r^{t'}(s^{t'},a^{t'})$.
However, due to the high variance of $R(t)$, the critic function
$Q_{\psi}(s_{t},a_{t})$ is used instead. 
\begin{equation}
Q_{\psi}(s_{t},a_{t})=\mathbb{E}_{a_{1}\sim\pi_{1},...,a_{N}\sim\pi_{N},s\sim T}[R(t)]
\end{equation}
The gradient $\nabla_{\theta}J(\pi_{\theta})$ is replaced as: 
\begin{equation}
\nabla_{\theta}J(\pi_{\theta})=\nabla_{\theta}\log(\pi_{\theta}(a_{t}|s_{t}))Q_{\psi}(s_{t},a_{t})
\end{equation}

The $Q_{\psi}(s_{t},a_{t})$ function is learned by minimizing the
TD loss: 
\begin{align}
\mathcal{L}_{Q}(\psi) & =\mathbb{E}_{(s,a,r,s')\sim D}\left[(Q_{\psi}(s,a)-y)^{2}\right]\label{eq:critic_target}\\
y & =r(s,a)+\psi\mathbb{E}_{a'\sim\pi(s')}[Q_{\Tilde{\psi}}(s',a')]
\end{align}
where $y$ is the target, $Q_{\Tilde{\psi}}$ is the target Q-value
function which is the value of previous Q-functions stored in the
replay buffer.

\textbf{Soft Actor-Critic} To avoid converging to the local minimum,
the entropy term $-\alpha\log\pi_{\theta}(a|s)$ is incorporated into the policy gradient:
\begin{align*}
\nabla_{\theta}J(\pi_{\theta}) & =\mathbb{E}_{s\sim D,a\sim\pi}\left[\nabla_{\theta}\log\pi_{\theta}(a|s)Q^{*}(a,s)\right]\\
Q^{*}(a,s) & =Q_{\psi}(s,a)-\alpha\log\pi_{\theta}(a|s)-b(s)
\end{align*}
where $b(s)$ is a state-dependent baseline, $\alpha>0$ is trade-off coefficient. Then the target $y$ in Eq.~(\ref{eq:critic_target})
is updated as: 
\begin{equation}
y=r(s,a)+\psi\mathbb{E}_{a'\sim\pi(s')}\left[Q_{\Tilde{\psi}}(s',a')-\alpha\log\pi_{\Tilde{\theta}}(a'|s')\right]
\end{equation}
where $\Tilde{\psi}$ and $\Tilde{\theta}$ are the network parameters
of the target critics and policies. 

\subsubsection{Multi-agent reinforcement learning (MARL)}

\label{sec:MARL} The multi-agent reinforcement learning framework
is described as Markov Decision game with a tuple $<N,S,\{O_{i}\}_{i\in N},\{A_{i}\}_{i\in N}>,P,\{R_{i}\}_{i\in N}>$,
where $N$ is the number of agent, $S$ is the set of state, $\{O_{i}\}_{i\in N}$
is the observation space of N agents, $\{A_{i}\}_{i\in N}$ is joint
action of N agents, and $\{R_{i}\}_{i\in N}$ is reward for each agents.
The agent $i$ chooses an action based on the policy function $\pi_{\theta_{i}}:O_{i}\rightarrow P(A_{i})$
where $P(A_{i})$ is the distribution over action set $A_{i}$ given
observation $O_{i}$. Then the state $s$ and joint action $A$ lead
to the next state $s'$ with the probability function $P$. The agent
$i$ receives a reward based on the state and action of other
agents $R_{i}:S\times\{A_{i}\}_{i\in N}$.



==> method_problem.tex <==
In this section, we first formulate the counterfactual generation for drug-target binding affinity problem. Then, we introduce the counterfactual generation for drug molecule using reinforcement learning. Next, we propose the protein counterfactual generation using reinforcement learning. Finally, we propose the multi-agent reinforcement learning framework to combine drug and protein counterfactual generation.
\subsection{Drug-target counterfactual problem formulation}
Given the the drug $D$ and the target protein $P$, the counterfactual instance of drug-target complex ($D-P$) is the drug $\mathcal{\Tilde{D}} = D + \Delta D$ and the target protein $\mathcal{\Tilde{P}} = P + \Delta P$. 

We denote the drug-target binding affinity prediction model as:
\begin{equation}
A=\mathcal{F}_{\theta}(P,D),
\end{equation}

The counterfactual instance of the drug-target complex satisfies two properties: the substantial change in the binding affinity and minimizing the change in drug and target protein. Therefore, the counterfactual instance generation can be formulated as maximization problem:
\begin{equation}
    \argmax_{\Tilde{D}, \Tilde{P}} \mathcal{L}(\mathcal{F}_{\theta}(P,\mathcal{D}), \mathcal{F}_{\theta}(\Tilde{P},\Tilde{D})) + \mathcal{K}(P,\mathcal{\Tilde{P}}) + \mathcal{K}(D,\mathcal{\Tilde{D}})
\end{equation}

where K is the similarity function.
